Gaining Insights into Unrecognized User Utterances in Task-Oriented Dialog Systems

The rapidly growing market demand for automatic dialogue agents capable of goal-oriented behavior has caused many tech-industry leaders to invest considerable efforts into task-oriented dialog systems. The success of these systems is highly dependent on the accuracy of their intent identification -- the process of deducing the goal or meaning of the user's request and mapping it to one of the known intents for further processing. Gaining insights into unrecognized utterances -- user requests the systems fail to attribute to a known intent -- is therefore a key process in continuous improvement of goal-oriented dialog systems. We present an end-to-end pipeline for processing unrecognized user utterances, deployed in a real-world, commercial task-oriented dialog system, including a specifically-tailored clustering algorithm, a novel approach to cluster representative extraction, and cluster naming. We evaluated the proposed components, demonstrating their benefits in the analysis of unrecognized user requests.

==> chapters/2-related-work.tex <==
\section{Related Work}
\label{sec:rel-work}

In the context of the pipeline approach to building goal-oriented dialog systems, our work is related to the task of intent detection, performed by the NLU component. Intent detection is normally formulated as a standalone classification task \citep{xu2013convolutional, guo2014joint, chen2019bert}, which is loosely interlaced with the successive tasks in the pipeline. Out-of-domain utterance detection, which is the task of accurately discriminating between requests that are within- and outside the scope of a system, has gained much attention recently \citep{schuster2019cross, larson2019evaluation, gangal2020likelihood, cavalin2020improving}. Contrary to these works, we assume a set of utterances already labeled by a system's NLU module as unrecognized; these are user requests that the system failed to attribute to an existing intent. We demonstrate an end-to-end approach for extracting potentially actionable insights from these utterances, by making them easily accessible to a conversation analyst. 

Clustering is one of the most useful techniques for extracting insights from data in an unsupervised manner. In the context of text, clustering typically refers to the task of grouping together units (e.g., sentences, paragraphs, documents) carrying similar semantics, such that units in the same cluster are more semantically similar to each other than those in different clusters.
%
The unique nature of our setting imposes two constraints on the clustering algorithm: (1) unknown number of partitions, and (2) tolerating \textit{outliers} that lie isolated in low-density regions. Density-Based Spatial Clustering of Applications with Noise (DBSCAN) \citep{ester1996density} and its hierarchical version (HDBSCAN) \cite{mcinnes2017hdbscan} are two common choices that satisfy these requirements. We evaluate our clustering approach against (H)DBSCAN and show its benefits across multiple datasets. 

Another popular clustering algorithm that determines the number of partitions is MeanShift \citep{cheng1995mean}, a non-parametric method for locating the maxima of a density function. Outlier detection can further be achieved with MeanShift by considering only clusters that exceed a predefined minimal size, where the rest are assigned to the outlier pool. MeanShift yielded inferior performance in all our experiments; we, therefore, exclude its results from this work.



==> chapters/8-limitations.tex <==
\section{Limitations}
\label{sec:limitations}

The proposed clustering algorithm may entail efficiency considerations for a very large amount of data. As such, with pre-computed request embeddings, clustering time can reach a few minutes for batches of requests larger than $100$K.


==> chapters/9-appendices.tex <==
\appendix
\section{Appendices}
\subsection{Raduis-based Clustering Algorithm}
\label{sec:appendix-a}

\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\SetKwComment{Comment}{/*}{*/}

\begin{algorithm}
\caption{Radius-based Clustering}
\label{alg:clustering}
\SetInd{0.75em}{0.25em}
\small

\textbf{input}: {E (e1, e2, ... en)} \Comment{\hspace{0.05cm} elements}
%\textbf{input}: {D (n{$\times$}n)} \Comment{\hspace{0.05cm} dist matrix}
\textbf{input}: {min\_sim} \Comment{\hspace{0.05cm} min similarity}
\textbf{input}: {min\_size} \Comment{\hspace{0.05cm} min cluster size}
\BlankLine

$C \gets \emptyset$

\While{convergence criteria are not met}{
    \BlankLine
    \For{each element $e_i{\in}E$} {
        \BlankLine
        \eIf{the highest similarity of $e_i$ to any existing cluster exceeds min\_sim}{
            \BlankLine
            assign $e_i$ to its most similar cluster $c$ \\
            re-calculate the centroid of $c$
            \BlankLine
        }{
            \BlankLine
            create a new cluster $c^\prime$ and assign $e_i$ to it \\
            set the centroid of $c^\prime$ to be $e_i$ \\
            add $c^\prime$ to $C$
            \BlankLine
            
        }
    }
}
\BlankLine
\Comment{clusters with fewer elements than the predefined $min\_size$ are considered outliers}
\BlankLine
\textbf{return}: each $c{\in}C$ of size exceeding $min\_size$

\end{algorithm}


\subsection{Keyword-based Merging}
\label{sec:appendix-b}

%\paragraph{Keyword-based Merging}
User requests to a goal-oriented dialog system are likely to be characterized by the extensive use of a domain-specific lexicon. For example, in the domain of banking, we are likely to encounter terms related to `accounts', `transactions', and `balance', while in the context of a Covid-19 Q\&A bot, the lexicon is likely to contain extensive use of words related to `vaccine', `boosters', `appointments', and so on. Although impressive at capturing meaning, semantic representations do not necessarily capture the domain-specific notion of similar requests. For example, the two utterances `covid 19 and pregnancy' and `7 months pregnant and tested positive for covid, any risks?' do not exhibit exceptional semantic similarity, while practically they should be clustered together. The intuition that stems from the fact that both sentences contain `pregnant'/`pregnancy', and `covid' -- words typical of the underlying domain. We therefore suggest the additional, keyword-based merging approach, as detailed below.

%\paragraph{Domain-specific Keywords Extraction} 
A common way to extract lexical characteristics of a corpus is using a \textit{log-odds ratio with informative Dirichlet prior} \citep{monroe2008fightin} -- a method that discovers markers with excessive frequency in one dataset compared to another. We used the collection of unhandled utterances as our target corpus and a random sample of $100$K sentences from a Wikipedia dump\footnote{We used the Wikipedia 2006 dump available at \url{https://nlp.lsi.upc.edu/wikicorpus/}.} as our background neutral dataset. Setting the strict log-odds score of \text{-}$5$, markers identified for the dataset of Covid-19 requests included \{`quarantine', `measures', `emergency', `pregnant', `sick', `leave', `risk'\}.

%\paragraph{Cluster Similarity Computation} 
Given a set of markers, we now define cluster similarity as follows: we denote the set of domain-specific markers discovered by the log-odds ratio procedure by ${M}$ and the set of top-k most frequent words\footnote{k=$10$ by qualitative evaluation over the $[3, 15]$ range.} in two clusters $c_1$ and $c_2$, by ${W}_1$ and ${W}_2$, respectively. The similarity of $c_1$ and $c_2$ is then defined to be proportional to the number of markers from ${M}$ that can be found in both ${W}_1$ and ${W}_2$: $sim(c_1, c_2) \propto |{M} \cap {W}_1 \cap {W}_2|$, where $|{M}|$ amounts to the maximal possible similarity. Pairwise cluster distances are further computed by normalizing the similarity values to the $[0, 1]$ range, and subtracting them from $1$. A distance matrix $D_c$ is constructed by calculating pairwise distance on the set of clusters in ${C}$, and is further used as an input to a subsequent invocation of the RBC algorithm, with an adjusted \textit{min\_sim} threshold.

Following this definition and assuming a sample set of domain-specific markers \{`covid', `risk', `quarantine', `pregnant', `appointment', `test', `positive'\}, the two utterances `covid 19 and pregnancy' and `7 months pregnant and tested positive for covid, any risks?' will exhibit considerable keyword-based similarity (intersection size{=}2), despite only moderate semantic proximity.
